TSLA: A Task-Specific Learning Adaptation for Semantic Segmentation on Autonomous Vehicles Platform

Autonomous driving platforms encounter diverse driving scenarios, each with varying hardware resources and precision requirements. Given the computational limitations of embedded devices, it is crucial to consider computing costs when deploying on target platforms like the NVIDIA\textsuperscript{\textregistered} DRIVE PX 2. Our objective is to customize the semantic segmentation network according to the computing power and specific scenarios of autonomous driving hardware. We implement dynamic adaptability through a three-tier control mechanism -- width multiplier, classifier depth, and classifier kernel -- allowing fine-grained control over model components based on hardware constraints and task requirements. This adaptability facilitates broad model scaling, targeted refinement of the final layers, and scenario-specific optimization of kernel sizes, leading to improved resource allocation and performance. Additionally, we leverage Bayesian Optimization with surrogate modeling to efficiently explore hyperparameter spaces under tight computational budgets. Our approach addresses scenario-specific and task-specific requirements through automatic parameter search, accommodating the unique computational complexity and accuracy needs of autonomous driving. It scales its Multiply-Accumulate Operations (MACs) for Task-Specific Learning Adaptation (TSLA), resulting in alternative configurations tailored to diverse self-driving tasks. These TSLA customizations maximize computational capacity and model accuracy, optimizing hardware utilization.

==> sections/8-authors.tex <==


% \vspace{-2cm}


% \vspace{-4cm}



\begin{IEEEbiography}

[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/junliu.png}}]{Jun Liu}
is a PhD student under the supervision of Professor Yanzhi Wang in computer engineering at Northeastern University, Boston, MA. He is also a researcher at the Robotics Institute at Carnegie Mellon University in Pittsburgh, PA.
He received his Bachelor's and Master’s degrees from Beihang University, Beijing, China.
His current research interests include efficient AI, 3D wireless perception, software/hardware co-design, Computer Vision, and LLM (Large Language Model).\end{IEEEbiography}
\vspace{-1cm}






\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/zhenglun.png}}]{Zhenglun Kong}
is a PhD student at Northeastern University, supervised by Prof. Yanzhi Wang. He received his master degree from Northeastern University in 2019 and B.E. degree from Huazhong University of Science and Technology (HUST), China, in 2017.  He was a research intern at Microsoft Research. His research focuses on developing efficient deep learning methods applicable to real-world scenarios, including computer vision and natural language processing.\end{IEEEbiography}
\vspace{-1cm}


\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/weihao.jpg}}]{Weihao Zeng}
is currently a Machine Learning Engineer at Tesla Autopilot, working on Full Self-Driving (FSD) planning. He holds a Master's in Robotics from Carnegie Mellon University. He completed his Master's in Robotics at Carnegie Mellon University, under the supervision of Prof. Katia Sycara. His research interests are in Machine Learning, Reinforcement Learning, Autonomous Vehicles, and Computer Vision.\end{IEEEbiography}
\vspace{-1.0cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/changdi.jpg}}]{Changdi Yang}
received his BS degree from China Agricultural University, Beijing, China, in 2019. He is currently working toward a PhD degree under the supervision of Professor Yanzhi Wang in computer engineering at Northeastern University, Boston, MA. His current research interests include efficient deep learning, computer vision and trustworthy and explainable AI.\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/pu.jpg}}]{Pu Zhao}
is a research assistant professor at Northeastern University, Boston, MA. He received his Ph.D. degree in Computer Engineering from Northeastern University. Before that, he received his Bachelor's and Master’s degrees from Shanghai Jiao Tong University, Shanghai, China. His research interests include LLM (Large Language Model), AIGC (AI Generated Content), efficient AI, robust AI, and deep learning. \end{IEEEbiography}
% \vspace{-3cm}
\vspace{-1cm}



\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/xuan.jpeg}}]{Xuan Shen}
is a PhD student under the supervision of Professor Yanzhi Wang in computer engineering at Northeastern University, Boston, MA.
He received a B.S. in statistics from Nanjing University of Science and Technology, Nanjing, China 2018.
His current research interests include AIGC (AI-generated content), efficient AI, software/hardware co-design, and deep learning theory.\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/hao.png}}]{Hao Tang}
is a postdoctoral fellow at Carnegie Mellon University, USA. 
Before that, he held a postdoctoral position at ETH Zürich, Switzerland. He earned a master's degree from Peking University, China, and Ph.D. from the University of Trento, Italy.
He was a visiting scholar at the University of Oxford, UK. 
His research interests include AIGC, AI4Science, machine learning, computer vision, embodied AI, and the applications of such tools to scientific domains. \end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/wenbin.png}}]{Wenbin Zhang}
is an Assistant Professor at the Knight Foundation School of Computing \& Information Sciences at Florida International University, and an Associate Member at the Te Ipu o te Mahara Artificial Intelligence Institute. His research investigates the theoretical foundations of machine learning with a focus on societal impact and welfare. In addition, he has worked in a number of application areas, highlighted by work on transportation and healthcare. He is a recipient of best paper awards/candidates at FAccT’23, ICDM’23, DAMI, and ICDM’21, as well as the NSF CRII Award and recognition in the AAAI’24 New Faculty Highlights.
\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/geng.png}}]{Geng Yuan}
 is an assistant professor, at the  School of Computing (CS Department) at the University of Georgia. He received his Ph.D. Degree in Computer Engineering from Northeastern University (NEU) in 2023, under the supervision of Prof. Yanzhi Wang.
His research interests are in general AI systems, including energy-efficient deep learning and artificial intelligence systems, efficient training, model compression, hardware-software co-design for DNN architectures, and emerging deep learning systems.\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/wei.jpg}}]{Wei Niu}
is an assistant professor in the School of Computing at the University of Georgia. He obtained his Ph.D. degree from the Department of Computer Science at William \& Mary, under the supervision of Dr. Bin Ren. Prior to that, he earned a B.S. Degree in Software Engineering from Beihang University in 2016.
His research interests include Real-time machine learning systems, AGI on embedded devices, Parallel computing, Compiler optimization.\end{IEEEbiography}
\vspace{-0.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/xue.jpg}}]{Xue Lin}
is an associate professor in the Department of Electrical and Computer Engineering at Northeastern University. She received her bachelor’s degree in Microelectronics from Tsinghua University, China and her PhD degree from the Department of Electrical Engineering at University of Southern California in 2016. Her research interests include deep learning, machine learning and computing in cyber-physical systems, high-performance and mobile computing systems, and VLSI. Her research work has been recognized by multiple NSF awards and supported by Air Force Research Lab, Office of Naval Research, Lawrence Livermore National Lab, DARPA, and U.S. Department of Transportation.\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/yanzhi.png}}]{Yanzhi Wang}
(Member, IEEE) is currently an associate professor and faculty fellow at Dept. of ECE at Northeastern University, Boston, MA. He received the B.S. degree from Tsinghua University in 2009, and Ph.D. degree from University of Southern California in 2014. His research interests focus on model compression and platform specific acceleration of deep learning applications. He has received the U.S. Army Young Investigator Program Award (YIP), IEEE TC-SDM Early Career Award, Massachusetts Acorn Innovation Award, Martin Essigmann Excellence in Teaching Award, Massachusetts Acorn Innovation Award, Ming Hsieh Scholar Award, and other research awards from Google, MathWorks, etc. \end{IEEEbiography}





